Do Earth-Trained Humanoid Controllers Walk on the Moon? Gravity, Terrain, and Soil Transfer

Humanoid robots could aid lunar operations, but how to train their locomotion controllers for lunar gravity, terrain, and soil is unclear. We compare 12 strategies for a simulated Unitree G1 across gravity, terrain, and rigid or granular 3D resistive force theory (3D RFT) contact. Earth-trained policies keep 0.64 to 0.75 survival at the Moon on flat rigid ground in 10 s episodes, but falls continue, so longer episodes would see lower survival. Moon-trained and fine-tuned policies, in contrast, fall in every Earth episode, nearly all within 2 s. Rough-terrain training helps on uneven rigid ground only at training gravity. 3D RFT soil training helps on Earth sand but little on lunar soil. On three held-out soil models, Moon-trained policies lose no detectable progress at lunar gravity. Among tested strategies, only gravity-randomized rough 3D RFT training keeps mean survival above 0.83 at Earth and 0.95 at the Moon on all key tests up to 20 deg. Its ablation without soil training differs consistently only on soil at Earth gravity, falling in most sand episodes. These predictions depend on the contact model and soil stiffness, so lunar soil claims require agreement across soil models.

==> sections/5c-hardware.tex <==
\section{Scope of Physical Validation}
\label{sec:hardware}
\label{sec:res_earth}

The lab platform is Fauna Sprout, whereas the present simulation study uses Unitree G1. Sprout's technical report describes custom low-level policy deployment, actuator models, and robot descriptions~\cite{fauna_sprout_2026}. Availability in the lab SDK remains to be confirmed. Physical Sprout trials cannot directly validate G1 deployment or its predicted operating envelope. Hardware validation is therefore a conditional extension, requiring a matched Sprout model and controller before any simulator--hardware comparison. A demonstration with Sprout's supplied controller alone would be a separate embodiment/controller test.

If that extension is pursued, the same Sprout checkpoint is evaluated on rigid floor and a characterized dry-sand bed in hardware and simulation. Commands and horizon must be feasible for Sprout and the physical bed. Overhead position/heading measurements and synchronized joint/inertial logs provide progress and contact-related observables. Bed preparation, compaction, and reset procedures are recorded between trials. Density, friction, cohesion, plate loading, and lateral intrusion characterize the bed independently of the held-out walking trials. \todo{freeze horizon, repetitions, calibration/validation split, and measurement uncertainties; characterize model-specific parameters rather than setting only similarly named material fields}

\begin{table}[!tb]
  \centering\footnotesize
  \caption{\bfseries Conditional Sprout validation. Compare each engine's floor-to-sand change with the same embodiment and controller in hardware. A dash denotes a pending measurement, not a completed result. The engines are the material point method (MPM), soil contact model (SCM), and continuous representation model (CRM).}
  \label{tab:hardware}
  \setlength{\tabcolsep}{3pt}
  \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}|l|c|ccc|}
    \hline
    \textbf{Observable} & \textbf{Hardware} & \textbf{MPM} & \textbf{SCM} & \textbf{CRM$^*$} \\
    \hline\hline
    Completion change & -- & -- & -- & -- \\
    Forward speed change [m/s] & -- & -- & -- & -- \\
    Lateral deviation change [m] & -- & -- & -- & -- \\
    Final heading change [rad] & -- & -- & -- & -- \\
    Residual footprint depth [cm] & -- & -- & -- & -- \\
    \hline
  \end{tabular*}
  \par\smallskip $^*$After corrected contact behavior is characterized.
\end{table}

\todo{report absolute floor and sand outcomes as well as paired changes, per deployed checkpoint; use independently calibrated material parameters and matching heading feedback in simulation}
\todo{include work/energy only if measured quantities permit a defensible comparison. Estimated joint work and electrical energy are distinct; commanded torque is not measured torque}
\todo{state which observables agree with Earth measurements, with uncertainty and tested conditions. Earth agreement constrains those predictions but does not select a validated lunar model}


==> sections/5d-largescale.tex <==
% Supplementary source: deliberately excluded from body.tex.
\section{Local Transfer on DEM-Based Terrain}
\label{sec:largescale}
The historical deployment evaluates 16 paired starts on a fixed $4\times4$ grid with \SI{12}{\metre} spacing on one local patch of an OmniLRS-based environment~\cite{rodriguez_omnilrs_2023}. The \SI{5}{\metre} per pixel Lunar Orbiter Laser Altimeter (LOLA) DEM supplies regional relief~\cite{barker_improved_2021}. Walking-scale geometry is procedural. These starts do not exercise extensive traversal or establish geographically broad lunar robustness.

\todo{if retained: verify the common policy interface, pair locations and headings across policies, record endpoints and paths, and report commanded forward progress rather than distance alone. Keep historical policy results separate from the new study}
\todo{replace the historical terrain gallery with current collision-geometry profiles, foot dimensions, and actual evaluated trajectories. The prior posed robot image and obsolete CRM surface panel are illustrations, not evidence for current locomotion or comparative sinkage}


==> tables/tab_earthregolith.tex <==
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}|l|cc|cc|}
\hline
& \multicolumn{2}{c|}{\textbf{Earth sand}} & \multicolumn{2}{c|}{\textbf{Lunar regolith}} \\
\hdrstrut \textbf{Policy} & Flat & Comb. & Flat & Comb. \\
\hline\hline
\EarthFlatRigid & 0.96\,{\tiny[0.92,0.99]} & 0.27\,{\tiny[0.22,0.34]} & 0.99\,{\tiny[0.98,1.00]} & 0.38\,{\tiny[0.34,0.41]} \\
\EarthFlatRFT & 1.00 & 0.69\,{\tiny[0.61,0.76]} & 1.00 & 0.68\,{\tiny[0.62,0.73]} \\
\EarthRoughRigid & 0.33\,{\tiny[0.11,0.54]} & 0.30\,{\tiny[0.20,0.43]} & 1.00 & 0.98\,{\tiny[0.97,0.99]} \\
\EarthRoughRFT & 0.99\,{\tiny[0.98,1.00]} & 0.87\,{\tiny[0.72,0.95]} & 1.00 & 0.98\,{\tiny[0.97,0.98]} \\
\hline
\end{tabular*}


==> tables/tab_perprofile.tex <==
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}|l|cccccccc|}
\hline
\hdrstrut \textbf{Policy} & Fwd 0.25 & Fwd 0.5 & Fwd 1.0 & Bwd 0.5 & Side 0.3 & Turn & Step up & Step stop \\
\hline\hline
\multicolumn{9}{|l|}{\textbf{At Earth}} \\ \hline
\EarthFlatRigid & 0.90\,{\tiny[0.81,0.97]} & 0.57\,{\tiny[0.56,0.59]} & 0.17\,{\tiny[0.09,0.25]} & 0.72\,{\tiny[0.66,0.81]} & 0.75\,{\tiny[0.66,0.84]} & 0.49\,{\tiny[0.47,0.53]} & 0.26\,{\tiny[0.19,0.31]} & 0.36\,{\tiny[0.28,0.41]} \\
\EarthFlatRFT & 0.89\,{\tiny[0.81,0.97]} & 0.74\,{\tiny[0.62,0.91]} & 0.50\,{\tiny[0.38,0.59]} & 0.73\,{\tiny[0.66,0.84]} & 0.80\,{\tiny[0.66,0.91]} & 0.66\,{\tiny[0.56,0.72]} & 0.62\,{\tiny[0.56,0.69]} & 0.64\,{\tiny[0.53,0.72]} \\
\EarthRoughRigid & 1.00 & 0.96\,{\tiny[0.94,0.97]} & 0.97\,{\tiny[0.94,1.00]} & 1.00 & 1.00 & 0.99\,{\tiny[0.97,1.00]} & 0.96\,{\tiny[0.94,0.97]} & 1.00 \\
\EarthRoughRFT & 1.00 & 0.95\,{\tiny[0.91,1.00]} & 0.94\,{\tiny[0.91,0.97]} & 1.00 & 0.98\,{\tiny[0.97,1.00]} & 1.00 & 0.95\,{\tiny[0.91,0.97]} & 0.99\,{\tiny[0.97,1.00]} \\
\hline
\MoonFlatRigid & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
\MoonFlatRFT & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
\MoonRoughRigid & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
\MoonRoughRFT & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
\hline
\FtFlatRigid & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
\FtRoughRFT & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
\JointFlatRigid & 0.61\,{\tiny[0.53,0.69]} & 0.18\,{\tiny[0.09,0.34]} & 0.09\,{\tiny[0.06,0.12]} & 0.52\,{\tiny[0.44,0.56]} & 0.60\,{\tiny[0.50,0.78]} & 0.17\,{\tiny[0.03,0.25]} & 0.07\,{\tiny[0.03,0.09]} & 0.08\,{\tiny[0.06,0.12]} \\
\JointRoughRFT & 0.97 & 0.95\,{\tiny[0.91,0.97]} & 0.90\,{\tiny[0.84,0.94]} & 0.99\,{\tiny[0.97,1.00]} & 0.97\,{\tiny[0.94,1.00]} & 1.00 & 0.92\,{\tiny[0.88,0.97]} & 0.94\,{\tiny[0.91,0.97]} \\
\hline
\multicolumn{9}{|l|}{\textbf{At Moon}} \\ \hline
\EarthFlatRigid & 0.79\,{\tiny[0.72,0.84]} & 0.38\,{\tiny[0.31,0.44]} & 0.19\,{\tiny[0.09,0.25]} & 0.44\,{\tiny[0.28,0.62]} & 0.64\,{\tiny[0.56,0.69]} & 0.33\,{\tiny[0.22,0.44]} & 0.58\,{\tiny[0.50,0.62]} & 0.22\,{\tiny[0.06,0.34]} \\
\EarthFlatRFT & 0.71\,{\tiny[0.56,0.88]} & 0.40\,{\tiny[0.25,0.56]} & 0.35\,{\tiny[0.28,0.50]} & 0.30\,{\tiny[0.19,0.44]} & 0.69\,{\tiny[0.59,0.81]} & 0.33\,{\tiny[0.19,0.44]} & 0.45\,{\tiny[0.41,0.47]} & 0.24\,{\tiny[0.09,0.41]} \\
\EarthRoughRigid & 0.43\,{\tiny[0.16,0.69]} & 0.48\,{\tiny[0.34,0.66]} & 0.55\,{\tiny[0.53,0.56]} & 0.21\,{\tiny[0.09,0.34]} & 0.41\,{\tiny[0.25,0.59]} & 0.42\,{\tiny[0.31,0.59]} & 0.60\,{\tiny[0.41,0.84]} & 0.35\,{\tiny[0.31,0.38]} \\
\EarthRoughRFT & 0.57\,{\tiny[0.41,0.75]} & 0.59\,{\tiny[0.47,0.81]} & 0.67\,{\tiny[0.53,0.88]} & 0.38\,{\tiny[0.12,0.50]} & 0.45\,{\tiny[0.22,0.56]} & 0.51\,{\tiny[0.31,0.88]} & 0.61\,{\tiny[0.44,0.81]} & 0.55\,{\tiny[0.41,0.75]} \\
\hline
\MoonFlatRigid & 0.93\,{\tiny[0.88,0.97]} & 0.85\,{\tiny[0.78,0.94]} & 0.62\,{\tiny[0.56,0.72]} & 0.90\,{\tiny[0.88,0.91]} & 0.95\,{\tiny[0.88,1.00]} & 0.82\,{\tiny[0.75,0.91]} & 0.69\,{\tiny[0.66,0.72]} & 0.68\,{\tiny[0.59,0.72]} \\
\MoonFlatRFT & 0.89\,{\tiny[0.88,0.91]} & 0.81 & 0.44\,{\tiny[0.28,0.59]} & 0.95\,{\tiny[0.84,1.00]} & 0.98\,{\tiny[0.94,1.00]} & 0.80\,{\tiny[0.75,0.84]} & 0.53\,{\tiny[0.50,0.56]} & 0.49\,{\tiny[0.38,0.66]} \\
\MoonRoughRigid & 0.99\,{\tiny[0.97,1.00]} & 1.00 & 0.98\,{\tiny[0.97,1.00]} & 0.97 & 0.97\,{\tiny[0.94,1.00]} & 1.00 & 1.00 & 1.00 \\
\MoonRoughRFT & 0.99\,{\tiny[0.97,1.00]} & 0.97 & 0.91\,{\tiny[0.78,1.00]} & 1.00 & 1.00 & 0.98\,{\tiny[0.97,1.00]} & 0.98\,{\tiny[0.97,1.00]} & 0.94\,{\tiny[0.88,1.00]} \\
\hline
\FtFlatRigid & 0.95\,{\tiny[0.91,1.00]} & 0.93\,{\tiny[0.91,0.94]} & 0.68\,{\tiny[0.56,0.75]} & 0.95\,{\tiny[0.88,1.00]} & 0.97\,{\tiny[0.94,1.00]} & 0.89\,{\tiny[0.84,0.91]} & 0.68\,{\tiny[0.59,0.75]} & 0.70\,{\tiny[0.66,0.75]} \\
\FtRoughRFT & 0.99\,{\tiny[0.97,1.00]} & 0.97\,{\tiny[0.94,1.00]} & 0.96\,{\tiny[0.94,1.00]} & 0.99\,{\tiny[0.97,1.00]} & 0.99\,{\tiny[0.97,1.00]} & 0.99\,{\tiny[0.97,1.00]} & 1.00 & 0.96\,{\tiny[0.94,0.97]} \\
\JointFlatRigid & 0.69\,{\tiny[0.59,0.78]} & 0.46\,{\tiny[0.41,0.50]} & 0.21\,{\tiny[0.19,0.22]} & 0.90\,{\tiny[0.81,1.00]} & 0.85\,{\tiny[0.78,0.91]} & 0.51\,{\tiny[0.47,0.56]} & 0.41\,{\tiny[0.34,0.47]} & 0.25\,{\tiny[0.19,0.31]} \\
\JointRoughRFT & 1.00 & 0.99\,{\tiny[0.97,1.00]} & 1.00 & 1.00 & 1.00 & 0.99\,{\tiny[0.97,1.00]} & 0.99\,{\tiny[0.97,1.00]} & 0.97\,{\tiny[0.94,1.00]} \\
\hline
\end{tabular*}


==> tables/tab_perseed_route.tex <==
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}|l|c|cccc|cc|}
\hline
& & \multicolumn{4}{c|}{\textbf{Moon}} & \multicolumn{2}{c|}{\textbf{Earth}} \\
\hdrstrut \textbf{Policy} & \textbf{Seed} & $S\uparrow$ & $e_v\downarrow$ & $\rho_v^{\rm RFT}$ & $\rho_v^{\rm MPM}$ & $S\uparrow$ & $e_v\downarrow$ \\
\hline\hline
\MoonFlatRigid & 42 & 1.00 & 0.04 & -- & -- & 0.00 & -- \\
\MoonFlatRigid & 43 & 1.00 & 0.03 & -- & -- & 0.00 & -- \\
\MoonFlatRigid & 44 & 1.00 & 0.03 & -- & -- & 0.00 & -- \\
\hline
\FtFlatRigid & 42 & 1.00 & 0.03 & -- & -- & 0.00 & -- \\
\FtFlatRigid & 43 & 1.00 & 0.02 & -- & -- & 0.00 & -- \\
\FtFlatRigid & 44 & 1.00 & 0.02 & -- & -- & 0.00 & -- \\
\hline
\JointFlatRigid & 42 & 1.00 & 0.02 & -- & -- & 0.96 & 0.01 \\
\JointFlatRigid & 43 & 1.00 & 0.02 & -- & -- & 0.88 & 0.01 \\
\JointFlatRigid & 44 & 1.00 & 0.03 & -- & -- & 0.91 & 0.02 \\
\hline
\EarthFlatRigid & 42 & 0.70 & 0.15 & -- & -- & 1.00 & 0.01 \\
\EarthFlatRigid & 43 & 0.56 & 0.16 & -- & -- & 1.00 & 0.01 \\
\EarthFlatRigid & 44 & 0.66 & 0.18 & -- & -- & 1.00 & 0.01 \\
\hline
\MoonRoughRFT & 42 & 0.99 & 0.08 & 1.04 & 1.15 & 0.00 & -- \\
\MoonRoughRFT & 43 & 0.97 & 0.12 & 1.03 & 1.04 & 0.00 & -- \\
\MoonRoughRFT & 44 & 0.95 & 0.11 & 1.18 & 0.89 & 0.00 & -- \\
\hline
\FtRoughRFT & 42 & 0.98 & 0.12 & 1.02 & 1.00 & 0.00 & -- \\
\FtRoughRFT & 43 & 0.98 & 0.09 & 1.04 & 0.94 & 0.00 & -- \\
\FtRoughRFT & 44 & 0.99 & 0.11 & 1.05 & 0.98 & 0.00 & -- \\
\hline
\JointRoughRFT & 42 & 1.00 & 0.11 & 1.07 & 1.09 & 0.96 & 0.07 \\
\JointRoughRFT & 43 & 0.99 & 0.10 & 1.04 & 0.95 & 0.94 & 0.05 \\
\JointRoughRFT & 44 & 0.99 & 0.10 & 1.02 & 0.88 & 0.96 & 0.08 \\
\hline
\EarthRoughRFT & 42 & 0.51 & 0.29 & 2.49 & --$^\dagger$ & 0.97 & 0.05 \\
\EarthRoughRFT & 43 & 0.74 & 0.28 & 1.20 & --$^\dagger$ & 0.97 & 0.04 \\
\EarthRoughRFT & 44 & 0.38 & 0.27 & 2.27 & --$^\dagger$ & 0.98 & 0.05 \\
\hline
\end{tabular*}


==> tables/tab_perseed_soil.tex <==
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}|l|c|cc|cc|cc|c|}
\hline
& & \multicolumn{2}{c|}{\textbf{3D RFT}} & \multicolumn{2}{c|}{\textbf{MPM}} & \multicolumn{2}{c|}{\textbf{SCM}} & \textbf{CRM} \\
\hdrstrut \textbf{Policy} & \textbf{Seed} & Flat & Comb. & Flat & Comb. & Flat & Comb. & Flat \\
\hline\hline
\EarthFlatRigid & 42 & 0.98 & 0.78 & 0.44 & 2.14 & 0.94 & 1.25 & 0.99 \\
\EarthFlatRigid & 43 & 1.09 & 0.81 & 0.89 & 1.07 & 0.95 & 1.36 & 0.98 \\
\EarthFlatRigid & 44 & 1.05 & 0.82 & 0.96 & 0.55 & 0.98 & 1.51 & 0.98 \\
\hline
\EarthFlatRFT & 42 & 1.05 & 0.93 & 1.07 & 1.07 & 1.05 & 1.33 & 1.06 \\
\EarthFlatRFT & 43 & 1.06 & 0.87 & 0.49 & 1.05 & 1.05 & 1.15 & 1.08 \\
\EarthFlatRFT & 44 & 1.08 & 0.91 & 1.04 & 1.59 & 1.05 & 1.06 & 1.07 \\
\hline
\EarthRoughRigid & 42 & 1.05 & 0.92 & 1.03 & 1.09 & 1.05 & 0.92 & 1.04 \\
\EarthRoughRigid & 43 & 1.11 & 0.97 & 1.03 & 0.99 & 1.06 & 0.90 & 1.03 \\
\EarthRoughRigid & 44 & 0.99 & 0.91 & 1.04 & 1.04 & 1.08 & 0.92 & 1.02 \\
\hline
\EarthRoughRFT & 42 & 0.87 & 0.89 & 1.02 & 0.97 & 0.96 & 0.93 & 1.08 \\
\EarthRoughRFT & 43 & 0.97 & 0.93 & 1.06 & 1.04 & 1.06 & 0.96 & 1.05 \\
\EarthRoughRFT & 44 & 0.97 & 0.96 & 1.10 & 1.03 & 1.05 & 0.95 & 1.08 \\
\hline
\MoonFlatRigid & 42 & 1.04 & 1.34 & 1.01 & 1.11 & 1.05 & 1.02 & 1.08 \\
\MoonFlatRigid & 43 & 1.04 & 1.39 & 0.99 & 1.02 & 1.04 & 0.97 & 1.09 \\
\MoonFlatRigid & 44 & 1.04 & 1.31 & 1.01 & 1.01 & 1.04 & 1.03 & 1.09 \\
\hline
\MoonFlatRFT & 42 & 1.07 & 1.43 & 1.00 & 1.03 & 1.02 & 1.04 & 1.00 \\
\MoonFlatRFT & 43 & 1.00 & 1.66 & 1.04 & 2.51 & 0.87 & 1.04 & 0.94 \\
\MoonFlatRFT & 44 & 0.95 & 1.29 & 0.96 & 0.93 & 1.00 & 1.08 & 0.95 \\
\hline
\MoonRoughRigid & 42 & 0.84 & 0.92 & 0.86 & 0.84 & 1.39 & 1.03 & 1.21 \\
\MoonRoughRigid & 43 & 0.82 & 0.69 & 0.88 & 0.91 & 1.11 & 0.89 & 1.09 \\
\MoonRoughRigid & 44 & 1.00 & 1.00 & 1.02 & 1.00 & 1.07 & 0.84 & 1.09 \\
\hline
\MoonRoughRFT & 42 & 1.02 & 1.04 & 1.04 & 1.15 & 1.03 & 0.98 & 0.99 \\
\MoonRoughRFT & 43 & 0.94 & 1.03 & 0.95 & 1.04 & 1.07 & 0.99 & 0.95 \\
\MoonRoughRFT & 44 & 1.45 & 1.18 & 1.06 & 0.89 & 1.05 & 1.01 & 1.08 \\
\hline
\end{tabular*}


==> tables/tab_perseed_terrain.tex <==
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}|l|l|c|ccccc|cc|ccc|}
\hline
& & & \multicolumn{5}{c|}{\textbf{Tiles, $S\uparrow$}} & \multicolumn{2}{c|}{\textbf{Mesh, $S\uparrow$}} & \multicolumn{3}{c|}{\textbf{Combined tiles}} \\
\hdrstrut \textbf{Policy} & \textbf{Test} & \textbf{Seed} & Flat & Crat. & Rock & Und. & Comb. & Up & Down & $e_v\downarrow$ & $v_\parallel/v_c$ & Slip \\
\hline\hline
\EarthFlatRigid & Earth & 42 & 1.00 & 0.98 & 0.98 & 0.52 & 0.50 & 0.62 & 1.00 & 0.11 & 0.51 & 0.08 \\
\EarthFlatRigid & Earth & 43 & 1.00 & 0.99 & 0.98 & 0.59 & 0.52 & 0.67 & 1.00 & 0.10 & 0.49 & 0.08 \\
\EarthFlatRigid & Earth & 44 & 1.00 & 0.98 & 0.98 & 0.60 & 0.56 & 0.92 & 1.00 & 0.09 & 0.55 & 0.08 \\
\hline
\EarthFlatRigid & Moon & 42 & 0.70 & 0.70 & 0.73 & 0.50 & 0.49 & 0.80 & 0.42 & 0.23 & 0.43 & 0.31 \\
\EarthFlatRigid & Moon & 43 & 0.56 & 0.57 & 0.57 & 0.34 & 0.34 & 0.51 & 0.19 & 0.26 & 0.20 & 0.31 \\
\EarthFlatRigid & Moon & 44 & 0.66 & 0.71 & 0.73 & 0.50 & 0.50 & 0.61 & 0.57 & 0.27 & 0.25 & 0.31 \\
\hline
\EarthRoughRigid & Earth & 42 & 1.00 & 1.00 & 1.00 & 1.00 & 0.98 & 1.00 & 1.00 & 0.04 & 0.93 & 0.10 \\
\EarthRoughRigid & Earth & 43 & 1.00 & 1.00 & 1.00 & 0.99 & 0.99 & 1.00 & 1.00 & 0.04 & 0.93 & 0.09 \\
\EarthRoughRigid & Earth & 44 & 1.00 & 1.00 & 1.00 & 0.99 & 0.98 & 1.00 & 1.00 & 0.04 & 0.96 & 0.10 \\
\hline
\EarthRoughRigid & Moon & 42 & 0.79 & 0.77 & 0.74 & 0.37 & 0.31 & 0.85 & 0.55 & 0.25 & $-$0.03 & 0.24 \\
\EarthRoughRigid & Moon & 43 & 0.80 & 0.79 & 0.82 & 0.55 & 0.55 & 0.76 & 0.59 & 0.26 & 0.18 & 0.21 \\
\EarthRoughRigid & Moon & 44 & 0.62 & 0.66 & 0.71 & 0.50 & 0.43 & 0.65 & 0.73 & 0.27 & 0.15 & 0.25 \\
\hline
\MoonFlatRigid & Earth & 42 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & -- & 0.00 & -- \\
\MoonFlatRigid & Earth & 43 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & -- & 0.00 & -- \\
\MoonFlatRigid & Earth & 44 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & -- & 0.00 & -- \\
\hline
\MoonFlatRigid & Moon & 42 & 1.00 & 1.00 & 1.00 & 0.83 & 0.77 & 0.84 & 0.96 & 0.08 & 0.73 & 0.15 \\
\MoonFlatRigid & Moon & 43 & 1.00 & 0.98 & 1.00 & 0.80 & 0.79 & 0.98 & 1.00 & 0.07 & 0.75 & 0.15 \\
\MoonFlatRigid & Moon & 44 & 1.00 & 1.00 & 1.00 & 0.91 & 0.86 & 1.00 & 0.99 & 0.09 & 0.77 & 0.19 \\
\hline
\MoonRoughRigid & Earth & 42 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & -- & 0.00 & -- \\
\MoonRoughRigid & Earth & 43 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & -- & 0.00 & -- \\
\MoonRoughRigid & Earth & 44 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & -- & 0.00 & -- \\
\hline
\MoonRoughRigid & Moon & 42 & 1.00 & 1.00 & 1.00 & 1.00 & 0.99 & 1.00 & 1.00 & 0.09 & 0.75 & 0.23 \\
\MoonRoughRigid & Moon & 43 & 1.00 & 1.00 & 1.00 & 0.99 & 0.98 & 1.00 & 0.58 & 0.10 & 0.75 & 0.16 \\
\MoonRoughRigid & Moon & 44 & 1.00 & 1.00 & 1.00 & 0.99 & 0.99 & 1.00 & 1.00 & 0.11 & 0.86 & 0.16 \\
\hline
\end{tabular*}


==> tables/tab_route.tex <==
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}|l|cccc|cc|cc|}
\hline
& \multicolumn{4}{c|}{\textbf{Moon}} & \multicolumn{2}{c|}{\textbf{Earth}} & \multicolumn{2}{c|}{\textbf{Total}} \\
\hdrstrut \textbf{Policy} & $S\uparrow$ & $e_v\downarrow$ & $\rho_v^{\rm RFT}$ & $\rho_v^{\rm MPM}$ & $S\uparrow$ & $e_v\downarrow$ & Iter. & Steps \\
\hline\hline
\MoonFlatRigid & 1.00 & 0.03 & -- & -- & 0.00 & -- & 10 & 0.98 \\
\FtFlatRigid & 1.00 & 0.03 & -- & -- & 0.00 & -- & 15 & 1.47 \\
\JointFlatRigid & 1.00 & 0.02 & -- & -- & 0.92 & 0.02 & 10 & 0.98 \\
\EarthFlatRigid & 0.64 & 0.16 & -- & -- & 1.00 & 0.01 & 10 & 0.98 \\
\hline
\MoonRoughRFT & 0.97 & 0.10 & 1.08 & 1.03 & 0.00 & -- & 10 & 0.98 \\
\FtRoughRFT & 0.98 & 0.11 & 1.04 & 0.97 & 0.00 & -- & 15 & 1.47 \\
\JointRoughRFT & 0.99 & 0.10 & 1.04 & 0.97 & 0.95 & 0.07 & 10 & 0.98 \\
\EarthRoughRFT & 0.54 & 0.28 & 1.99 & --$^\dagger$ & 0.98 & 0.05 & 10 & 0.98 \\
\hline
\end{tabular*}


==> tables/tab_soil_falls.tex <==
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}|l|ccc|ccc|}
\hline
& \multicolumn{3}{c|}{\textbf{Flat soil}} & \multicolumn{3}{c|}{\textbf{Combined tiles under soil}} \\
\hdrstrut \textbf{Policy} & Tilt & Height & Both & Tilt & Height & Both \\
\hline\hline
\EarthFlatRigid & 6 & 0 & 0 & 480 & 0 & 0 \\
\EarthFlatRFT & 0 & 0 & 0 & 245 & 0 & 0 \\
\EarthRoughRigid & 0 & 0 & 0 & 13 & 0 & 0 \\
\EarthRoughRFT & 0 & 0 & 0 & 16 & 0 & 0 \\
\hline
\MoonFlatRigid & 0 & 0 & 0 & 33 & 0 & 0 \\
\MoonFlatRFT & 1 & 0 & 0 & 29 & 0 & 0 \\
\MoonRoughRigid & 0 & 0 & 0 & 15 & 0 & 0 \\
\MoonRoughRFT & 0 & 0 & 0 & 3 & 0 & 0 \\
\hline
\end{tabular*}


==> tables/tab_soil_geometries.tex <==
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}|l|ccccc|}
\hline
\hdrstrut \textbf{Policy} & Flat & Crat. & Rock & Und. & Comb. \\
\hline\hline
\EarthFlatRigid & 0.96\,{\tiny[0.92,0.99]} & 0.90\,{\tiny[0.84,0.95]} & 0.87\,{\tiny[0.80,0.92]} & 0.32\,{\tiny[0.28,0.40]} & 0.27\,{\tiny[0.22,0.34]} \\
\EarthFlatRFT & 1.00 & 0.99\,{\tiny[0.99,1.00]} & 0.97\,{\tiny[0.95,0.99]} & 0.78\,{\tiny[0.71,0.83]} & 0.69\,{\tiny[0.61,0.76]} \\
\EarthRoughRigid & 0.33\,{\tiny[0.11,0.54]} & 0.33\,{\tiny[0.13,0.55]} & 0.33\,{\tiny[0.10,0.54]} & 0.28\,{\tiny[0.15,0.39]} & 0.30\,{\tiny[0.20,0.43]} \\
\EarthRoughRFT & 0.99\,{\tiny[0.98,1.00]} & 0.98\,{\tiny[0.95,1.00]} & 0.98\,{\tiny[0.96,1.00]} & 0.92\,{\tiny[0.79,0.99]} & 0.87\,{\tiny[0.72,0.95]} \\
\hline
\MoonFlatRigid & 1.00 & 1.00 & 0.99\,{\tiny[0.99,1.00]} & 0.98\,{\tiny[0.98,0.99]} & 0.96\,{\tiny[0.94,0.98]} \\
\MoonFlatRFT & 1.00 & 1.00 & 0.99\,{\tiny[0.98,0.99]} & 0.98\,{\tiny[0.97,0.99]} & 0.96\,{\tiny[0.94,0.98]} \\
\MoonRoughRigid & 1.00 & 1.00\,{\tiny[0.99,1.00]} & 1.00 & 0.98\,{\tiny[0.96,1.00]} & 0.98\,{\tiny[0.96,0.99]} \\
\MoonRoughRFT & 1.00 & 1.00 & 1.00 & 1.00\,{\tiny[0.99,1.00]} & 1.00\,{\tiny[0.99,1.00]} \\
\hline
\end{tabular*}


==> tables/tab_soil_vs_rigid.tex <==
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}|l|cc|cc|}
\hline
& \multicolumn{2}{c|}{\textbf{Survival change $\Delta S$}} & \multicolumn{2}{c|}{\textbf{CoT ratio}} \\
\hdrstrut \textbf{Policy} & Flat & Comb. & Flat & Comb. \\
\hline\hline
\EarthFlatRigid & $-$0.01\,{\tiny[$-$0.02,0.00]} & $-$0.15\,{\tiny[$-$0.16,$-$0.14]} & 1.56\,{\tiny[1.48,1.65]} & 1.56\,{\tiny[1.46,1.72]} \\
\EarthFlatRFT & 0.00\,{\tiny[0.00,0.01]} & $-$0.02\,{\tiny[$-$0.03,0.00]} & 1.49\,{\tiny[1.46,1.51]} & 1.63\,{\tiny[1.51,1.78]} \\
\EarthRoughRigid & 0.00 & 0.00\,{\tiny[$-$0.01,0.00]} & 1.64\,{\tiny[1.52,1.77]} & 2.33\,{\tiny[2.25,2.38]} \\
\EarthRoughRFT & 0.00 & 0.00\,{\tiny[0.00,0.01]} & 1.70\,{\tiny[1.59,1.89]} & 2.00\,{\tiny[1.92,2.10]} \\
\hline
\MoonFlatRigid & 0.00 & 0.15\,{\tiny[0.12,0.18]} & 1.02\,{\tiny[0.98,1.05]} & 0.52\,{\tiny[0.47,0.57]} \\
\MoonFlatRFT & 0.00\,{\tiny[0.00,0.01]} & 0.23\,{\tiny[0.18,0.28]} & 0.96\,{\tiny[0.90,0.99]} & 0.49\,{\tiny[0.46,0.51]} \\
\MoonRoughRigid & 0.00 & $-$0.01\,{\tiny[$-$0.02,0.00]} & 1.21\,{\tiny[1.08,1.31]} & 1.14\,{\tiny[0.93,1.50]} \\
\MoonRoughRFT & 0.05\,{\tiny[0.00,0.14]} & 0.03\,{\tiny[0.01,0.04]} & 0.88\,{\tiny[0.42,1.18]} & 0.72\,{\tiny[0.67,0.78]} \\
\hline
\end{tabular*}


==> tables/tab_soilrft_full.tex <==
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}|l|cc|cc|cc|c|}
\hline
& \multicolumn{2}{c|}{\textbf{3D RFT}} & \multicolumn{2}{c|}{\textbf{MPM}} & \multicolumn{2}{c|}{\textbf{SCM}} & \textbf{CRM} \\
\hdrstrut \textbf{Policy} & Flat & Comb. & Flat & Comb. & Flat & Comb. & Flat \\
\hline\hline
\EarthFlatRigid & 1.04\,{\tiny[0.98,1.09]} & 0.80\,{\tiny[0.78,0.82]} & 0.76\,{\tiny[0.44,0.96]} & 1.26\,{\tiny[0.55,2.14]} & 0.96\,{\tiny[0.94,0.98]} & 1.37\,{\tiny[1.25,1.51]} & 0.98\,{\tiny[0.98,0.99]} \\
\EarthFlatRFT & 1.07\,{\tiny[1.05,1.08]} & 0.91\,{\tiny[0.87,0.93]} & 0.86\,{\tiny[0.49,1.07]} & 1.24\,{\tiny[1.05,1.59]} & 1.05 & 1.18\,{\tiny[1.06,1.33]} & 1.07\,{\tiny[1.06,1.08]} \\
\EarthRoughRigid & 1.05\,{\tiny[0.99,1.11]} & 0.93\,{\tiny[0.91,0.97]} & 1.03\,{\tiny[1.03,1.04]} & 1.04\,{\tiny[0.99,1.09]} & 1.06\,{\tiny[1.05,1.08]} & 0.91\,{\tiny[0.90,0.92]} & 1.03\,{\tiny[1.02,1.04]} \\
\EarthRoughRFT & 0.94\,{\tiny[0.87,0.97]} & 0.93\,{\tiny[0.89,0.96]} & 1.06\,{\tiny[1.02,1.10]} & 1.02\,{\tiny[0.97,1.04]} & 1.03\,{\tiny[0.96,1.06]} & 0.95\,{\tiny[0.93,0.96]} & 1.07\,{\tiny[1.05,1.08]} \\
\hline
\MoonFlatRigid & 1.04 & 1.35\,{\tiny[1.31,1.39]} & 1.00\,{\tiny[0.99,1.01]} & 1.05\,{\tiny[1.01,1.11]} & 1.04\,{\tiny[1.04,1.05]} & 1.01\,{\tiny[0.97,1.03]} & 1.09\,{\tiny[1.08,1.09]} \\
\MoonFlatRFT & 1.01\,{\tiny[0.95,1.07]} & 1.46\,{\tiny[1.29,1.66]} & 1.00\,{\tiny[0.96,1.04]} & 1.49\,{\tiny[0.93,2.51]} & 0.96\,{\tiny[0.87,1.02]} & 1.05\,{\tiny[1.04,1.08]} & 0.97\,{\tiny[0.94,1.00]} \\
\MoonRoughRigid & 0.89\,{\tiny[0.82,1.00]} & 0.87\,{\tiny[0.69,1.00]} & 0.92\,{\tiny[0.86,1.02]} & 0.92\,{\tiny[0.84,1.00]} & 1.19\,{\tiny[1.07,1.39]} & 0.92\,{\tiny[0.84,1.03]} & 1.13\,{\tiny[1.09,1.21]} \\
\MoonRoughRFT & 1.14\,{\tiny[0.94,1.45]} & 1.08\,{\tiny[1.03,1.18]} & 1.01\,{\tiny[0.95,1.06]} & 1.03\,{\tiny[0.89,1.15]} & 1.05\,{\tiny[1.03,1.07]} & 0.99\,{\tiny[0.98,1.01]} & 1.01\,{\tiny[0.95,1.08]} \\
\hline
\end{tabular*}


==> tables/tab_terrain.tex <==
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}|l|l|ccccc|cc|c|}
\hline
& & \multicolumn{5}{c|}{\textbf{Tiles, $S\uparrow$}} & \multicolumn{2}{c|}{\textbf{Mesh, $S\uparrow$}} & \textbf{Comb.} \\
\hdrstrut \textbf{Policy} & \textbf{Test} & Flat & Crat. & Rock & Und. & Comb. & Up & Down & $e_v\downarrow$ \\
\hline\hline
\EarthFlatRigid & Earth & 1.00 & 0.98 & 0.98 & 0.57 & 0.53 & 0.74 & 1.00 & 0.10 \\
\EarthFlatRigid & Moon & 0.64 & 0.66 & 0.68 & 0.45 & 0.45 & 0.64 & 0.39 & 0.25 \\
\EarthRoughRigid & Earth & 1.00 & 1.00 & 1.00 & 0.99 & 0.98 & 1.00 & 1.00 & 0.04 \\
\EarthRoughRigid & Moon & 0.74 & 0.74 & 0.76 & 0.47 & 0.43 & 0.75 & 0.62 & 0.26 \\
\hline
\MoonFlatRigid & Earth & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & -- \\
\MoonFlatRigid & Moon & 1.00 & 0.99 & 1.00 & 0.85 & 0.80 & 0.94 & 0.98 & 0.08 \\
\MoonRoughRigid & Earth & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & -- \\
\MoonRoughRigid & Moon & 1.00 & 1.00 & 1.00 & 0.99 & 0.99 & 1.00 & 0.86 & 0.10 \\
\hline
SONIC & Earth & 1.00 & 1.00 & 1.00 & 0.91 & 0.90 & 1.00 & 1.00 & 0.20 \\
SONIC & Moon & 0.10 & 0.10 & 0.09 & 0.05 & 0.08 & 0.06 & 0.00 & 0.32 \\
\hline
\end{tabular*}

